D$^2$NeRF: Self-Supervised Decoupling of Dynamic and Static Objects from a Monocular Video

Given a monocular video, segmenting and decoupling dynamic objects while recovering the static environment is a widely studied problem in machine intelligence. Existing solutions usually approach this problem in the image domain, limiting their performance and understanding of the environment. We introduce Decoupled Dynamic Neural Radiance Field (D$^2$NeRF), a self-supervised approach that takes a monocular video and learns a 3D scene representation which decouples moving objects, including their shadows, from the static background. Our method represents the moving objects and the static background by two separate neural radiance fields with only one allowing for temporal changes. A naive implementation of this approach leads to the dynamic component taking over the static one as the representation of the former is inherently more general and prone to overfitting. To this end, we propose a novel loss to promote correct separation of phenomena. We further propose a shadow field network to detect and decouple dynamically moving shadows. We introduce a new dataset containing various dynamic objects and shadows and demonstrate that our method can achieve better performance than state-of-the-art approaches in decoupling dynamic and static 3D objects, occlusion and shadow removal, and image segmentation for moving objects.

==> Sections/Method_OLD.tex <==

% \AT{this entire paragraph reads as a repetition of the intro? A bit verbose.. use at most \textit{one} sentence to recap?}
% \todo{
% Given a monocular video captured from a freely moving hand-held camera, 
% % our method decouples object motion in the scene from the camera motion and simultaneously reconstructs models of dynamic objects and static environment without any mask supervision.
% our method decouples object motion in the scene by simultaneously reconstructing two separate neural radiance fields of dynamic objects and the static environment without any form of supervision on masks of the moving objects.
% Such motion-based and template-free scheme allows the challenging targets, such as non-rigid body, unusual objects, a mixture of dynamic and static objects, and shadows, to be accurately identified and disentangled.}


% decouples object motion in the scene by simultaneously reconstructing two separate neural radiance fields of dynamic objects

% The following section first describes the components of our method, consisted of a static NeRF and its extension on dynamic scene, HyperNeRF.
% We then elaborate on the optimization scheme of \NAME{}, including a skewed entropy loss to enforce separate geometry and control the learning of both components. Next, we introduce an additional shadow field network to allow more accurate dynamic shadow decoupling in the scene. 

% \subsection{Review of HyperNeRF: Topologically Varying Neural Radiance Field}

Given a \textit{monocular} video captured from a freely \textit{moving} hand-held camera, our method reconstructs a neural scene representation that decouples moving objects from the static environment, assuming a constant illumination and known camera poses (e.g. calibrated with COLMAP \cite{colmap}).
% 
As illustrated in \Figure{overview}, our method achieves this by learning \textit{separate} radiance fields for static and dynamic portions of the scene, and doing so in a fully self-supervised fashion.
% 
We describe our architecture (\Section{architecture}), detail our self-supervised losses (\Section{supervision}), and describe how, while shadows are not explicitly modeled by NeRFs, a simple technique for their effective removal is attainable (\Section{shadows}).


\subsection{Composite Neural Radiance Field}
\label{sec:architecture}
% 
% Our architecture consists of a static and a dynamic component, each models the time-independent and time-varying parts of the scene.
% \paragraph{Static component}
% 
The static component builds upon NeRF~\cite{NERF}, which represents the scene as continuous spatial-dependent density $\sigma$ and spatial-view-dependent radiance $\mathbf{c}$ using an multi-layer perceptron~$\mathcal{F}^S$:
% 
\begin{align}
\begin{rcases}
\sigma^S(\mathbf{x}) \in \mathbb{R}
\\
\mathbf{c}^S(\mathbf{x}, \mathbf{d}) \in \mathbb{R}^3
\end{rcases} 
=
\mathcal{F}^S(\mathbf{x}, \mathbf{d})
\label{eq:nerf}
\end{align}
% 
\at{where $\mathbf{x} \in \mathbb{R}^3$ is the spatial coordinate, 
and $\mathbf{d} \in \mathbb{R}^3, \|\mathbf{d}\|=1$ is the view direction.}
% 
% 
% \paragraph{Dynamic component}
% \AT{this is too much detail, not enough to understand the method, but enough to confuse the reader... better skip it?}
% The dynamic component adapts an extended time-varying NeRF, and therefore takes an additional time input and learns a 6D mapping to the density and radiance.
% We choose to build upon HyperNeRF \cite{hypernerf}, a dynamic NeRF representation that accurately models scenes with non-rigid motions and topological changes. HyperNeRF optimizes a set of per-frame latent deformation code and predicts a deformation field and a hyper ambient coordinate, which is then conditioned by an MLP to represent time-varying scenes.
\at{To model the dynamic components of a scene, we adapt HyperNeRF~\cite{hypernerf}, which accurately captures scenes with \textit{non-rigid} motion as well as \textit{topological changes}.
% \WW{I agree giving details about HyperNeRF could be confusing, but my idea was to highlight the complexity of it and explain it has more capacity/easier to overfit. Maybe briefly mention and point reader to HyperNeRF paper?}
% \AT{yes, pointing out ease of overfit is a good idea, see sentence below}
\at{But such increased representation power in our setting can be detrimental, leading the model to represent static portions of the scene as dynamic effects.}
For convenience, we denote it as a neural function $\mathcal{F}^D$:}
% \AT{should we add the inputs to the density and radiance? more clear...}
% \WW{both density and radiance is spatial-temporal-dependent, while radiance additionally depends on view direction. Not sure if we should state it again because we kinda did in above for the static component.}
% 
\begin{align}
\begin{rcases}
\sigma^D(\mathbf{x}, \time) \in \mathbb{R}
\\
\mathbf{c}^D(\mathbf{x}, \mathbf{d}, \time) \in \mathbb{R}^3
\end{rcases} 
=
\mathcal{F}^D(\mathbf{x}, \mathbf{d}, \time)
\label{eq:hypernerf}
\end{align}
% 
where $\time \in \mathbb{R}$ indicates time.
Given a camera ray $\mathbf{r} = \mathbf{o} + t\mathbf{d}$ originating from $\mathbf{o} \in \mathbb{R}^3$ and with direction $\mathbf{d}$, the two models are then composited to calculate the color $\hat{C}$ of the camera ray by integrating the radiance according to volumetric rendering within a pre-defined depth range $[t_n, t_f]$:
% \FZ{Hmm, the equation has no $\mathbf{r}$ or $\time$ on the RHS}
% \AT{implied by the ray parameterization? you can make this explicit.. $\sigma^S(t)\equiv \sigma^S(\mathbf{r}(t)), \mathbf{d}$}
% \FZ{I'd prefer consistent and explicit expressions for math equations:) Eq 1, 2, 3 should be consistent to show dependency of variables, especially we have a $\time$ in place }
% \AT{you have to choose a balance between verbosity, and clarity of exposition -- I am fine either ways, but choose carefully ;)}
% 
% where $\mathbf{x} \in \mathbb{R}^3$ is the spatial coordinate, $\mathbf{d} \in S^2$ is 2D view direction ($\mathbf{d} \in \mathbf{R}^3$ is the unit view direction vector \WW{which is better?}), $\psi \in \mathbb{R}$ is the 1D time frame, $\sigma \in \mathbb{R}$ is the volumetric density and $\mathbf{c} \in \mathbb{R}^3$ is the radiance.
% 
% \AT{lol, I don't think you need to patent a "sum" :) :)}
% \at{To compound dynamic and static components, we adapt the volume rendering equation developed by NeRF-W \cite{nerfw}}:
% 
% To render the scene containing both dynamic and static components, we adapt the :
% 
\begin{align}
\hat{C}(\mathbf{r}, \time) = \int_{t_n}^{t_f} T(t)&\left( \sigma^S(t) \cdot \mathbf{c}^S(t) + \sigma^D(t,\time) \cdot \mathbf{c}^D(t,\time) \right) \, dt
\label{eq:compositnerf}
\\
T(t) &= exp\left(-\int_{t_n}^{t} (\sigma^S(s) + \sigma^D(s,\time)) \, ds\right)
\end{align}
% 
where we simplify our notation as $\sigma(t)\equiv \sigma(\mathbf{r}(t))$ and $\mathbf{c}(t)\equiv \mathbf{c}(\mathbf{r}(t), \mathbf{d})$.
% \FZ{I'd prefer consistent and explicit expressions for math equations:) Eq 1, 2, 3 should be consistent to show dependency of variables, especially we have a $\time$ in place }
% \AT{done, more explicit now}
Note that, with such an additive decomposition, samples from either fields are capable of terminating the camera ray and occluding the other.


% \AT{if you don't use the quantities defined in the commented text below in your exposition (at least for now... you did not) just skip it and just cite the quadrature section of the original NeRF paper?}
% In practice, the integrals are approximated via numerical quadrature:
% % 
% \begin{equation}
% \begin{split}
% \hat{C}(\mathbf{r}) &= \sum_{i=1}^N T_i(\alpha^S_i \cdot \mathbf{c}^S_i + \alpha^D_i \cdot \mathbf{c}^D_i)
% \\
% \text{where } T_i &= exp(-\sum_{j=1}^{i-1} (\sigma^S_j + \sigma^D_j)\delta_j)
% \\
% \alpha^S_i &= 1 - exp(-\sigma^S_i\delta_i), \text{   }  \alpha^D_i = 1 - exp(-\sigma^D_i\delta_i)
% \end{split}
% \end{equation}
% % 
% $\delta_i$ is the distance between $i$-th sample and $(i+1)$-th sample.


\begin{comment}
Intuitively, each component represents a separate radiance field, where the \at{sample density correlates with the probability of the camera ray terminating at sample position.}\AT{this is wrong? that's transmittance}
Two radiance fields are composed together in an additive style, where samples from either fields are capable of terminating the camera ray and occluding the other. The accumulated transmittance $T_i$ is therefore calculated with the sum of two densities. Individual $\alpha$ values are used as weights of different radiance predicted by each component ($\mathbf{c}^S_i$ and $\mathbf{c}^D_i$) when rendering the pixel color. 
\end{comment}

\subsection{Supervision Losses}
\label{sec:supervision}
\TODO{summarize the paragraphs here?}\WW{Tried to write one, but there isn't much to talk about, and it's probably confusing without introducing $w$ first. Considering deleting it.}

\ww{To enforce a correct separation of dynamic and static radiance fields, we apply a binary entropy loss augmented with a novel skewness hyperparameter, as well as a ray regularization that encourages a cleaner dynamic component.}
\FZ{Alternatively, introduce the photometric loss first, briefly explain the issues of such a naive implementation to motivate the following regularization terms. I wrote one below}
% I think the overall loss should be introduced here. Briefly introduce each term before getting into details. A bit strange to discuss regularization before even introducing the photometric loss.}

\paragraph{Photometric Loss}
To find the correct parameters of the static (\Eq{nerf}) and dynamic (\Eq{hypernerf}) NeRF networks, we first apply a photometric loss to ensure that the output image sequences of the composite NeRF (\Eq{compositnerf}) align with the input video frames:
% 
\begin{equation}
    \mathcal{L}_p(\mathbf{r}, \time) = \|\hat{C}(\mathbf{r}, \time) - C(\mathbf{r}, \time)\|_2^2
    \label{eq:photometricloss}
\end{equation}
% 
where $C(\mathbf{r}, \time)$ indicates the true color of camera ray $\mathbf{r}$ at the time $\time$ obtained from input video frames. Nonetheless, the photometric loss alone does not guarantee a correct separation of dynamic and static radiance fields. 
The dynamic component can naturally take over the static counterpart by incorrectly assigning occupancy of static objects to dynamic NeRF.
% , as the representation of the dynamic NeRF is more general and thus prone to overfitting.
% \WW{Above sentence seems a bit repetitive, remove it? Also at this point we should motivate for general entropy loss, not skewed one. Without general entropy loss the separation cannot be achieved.}
To enforce a correct separation, we apply a binary entropy loss augmented with a novel skewness hyperparameter (\Eq{entropyloss}), as well as a ray regularization (\Eq{rayloss}) that encourages a cleaner assignment of occupancy.

% We first define a compositing weight of dynamic and static components, $w$, for each 4D point (3D spatial location and 1D time) as the ratio of dynamic component density against total density:
% \begin{equation}
% w = \frac{\sigma^D}{\sigma^D + \sigma^S}
% \end{equation}
% Therefore, value of $w$ should be $0$ or $1$ for all 4D samples.

\paragraph{Dynamic vs. Static Factorization}
As physical objects cannot co-exist at the same spatial location, a physically realistic solution should have any position in space \textit{either} occupied by a static component or a dynamic component, but \textit{not both}.
To promote this behavior we denote the spatial ratio of dynamic vs. static density as:
% 
\begin{equation}
w(\mathbf{x}, \time) = \frac{\sigma^D(\mathbf{x}, \time)}{\sigma^D(\mathbf{x}, \time) + \sigma^S(\mathbf{x})} \in [0,1]
\end{equation}
% 
and then penalize the deviation of this from a categorical $\{0,1\}$ distribution via a binary entropy loss~\cite{star}:
% \WW{I put the reference in, tho I'm still not sure if that's necessary. A binary entropy is very standard.}
% \AT{WARNING: entropy losses have a single term, but you have two, so it's binary entropy}
% 
\begin{align}
\mathcal{L}_b(\mathbf{r}, \time) = \int_{t_n}^{t_f} H_b&( w(\mathbf{r}(t), \time)) \: dt
\label{eq:unskewed_entropyloss}
\\
H_b&(x) = -(x \cdot log(x) + (1-x) \cdot log(1-x))
\label{eq:entropy}
\end{align}
% 
However, due to the strong expressive power of the dynamic networks (\Eq{hypernerf}), optimizing the loss (\Eq{unskewed_entropyloss}) leads to the technique modeling parts of the scene as dynamic, regardless of whether they are dynamic or static; see~\Figure{entropy}~(right).
To overcome this issue, we designed a \textit{skewed} entropy loss to bias our loss to \textit{slightly favor} static explanations of the scene with skewness hyper-parameter $k$, where as illustrated in~\Figure{entropy}~(left) $k>1$ attains the desired behavior:
% 
\begin{align}
\mathcal{L}_s(\mathbf{r}, \time) = \int_{t_n}^{t_f} H_b( w(\mathbf{r}(t), \time)^k ) \: dt
\label{eq:entropyloss}
\end{align}

% However, due to the strong expressive power of dynamic component, which has an additional degree of freedom through the time input as well as more capacity provided by the time latent code and the deformation field, it rapidly learns the high frequency parts in the scene regardless of the parts being dynamic or not.
% Hence, a naive entropy loss causes the dynamic component to take over the static and unnecessarily learns a a large portion of static background.
% Fig \ref{fig:entropy} shows an example where the original entropy loss leads to a failed scene decoupling.
% To overcome this issue, we instead use a skewed entropy loss that prefers static component over the dynamic 
% 
% \begin{equation}
% H_{s}(\mathbf{r}) = -\frac{1}{N}\sum_{i=1}^N (w_i^k log(w_i^k) + (1-w_i^k)log(1-w_i^k))
% \end{equation}
% where $k \in \mathbb{R}$ is a hyperparameter that defines the skewness, and a larger value causes the peak of entropy loss to skew towards $1$. The loss therefore encourages more samples with a composite density from both components to shift towards static side instead of dynamic. 
% Because the weights of both network components are initialized with the identical random scheme, the values of $w$ are around $0.5$ for all the samples. By shifting the peak from $0.5$ to a larger value, the dynamic component would immediately be encouraged to predict lower density during the first few iterations. Only when there exists training inputs that cannot be explained purely with the static component (i.e., time-varying objects), dynamic component would then be used to reduce the gap between the rendering and observation.
% it would be more difficult for a sample to be occupied by the dynamic component and easier for the static component. This prevents the dynamic component from suppressing the static component and including undesired static part during learning. However, 


\input{fig/skewedentropy}

\paragraph{Ray Regularization}
Choosing a large value of skewness $k$ causes the appearance of fuzzy floaters (low-density particles) in the static portion of the scene; see \Figure{entropy}~\at{($k=10$)}.
As it can be intuitively understood from \Figure{entropy}~(left), this is caused by the small gradients of $H_b(x^k)$ as $x$ approaches zero.
To mitigate this effect, and reduce fuzziness in the reconstruction, we penalize the maximum of $w$ along each camera ray:
% 
\begin{equation}
\mathcal{L}_r(\mathbf{r}, \time) = \max_{t \in [t_n,t_f]} w(\mathbf{r}(t), \time)
\label{eq:rayloss}
\end{equation}
% 
Such loss can be intuitively interpreted as constraining the dynamic component to occupy as few pixels as possible while minimizing the impact on the overall loss for all samples. Note that the purpose of $L_r(\mathbf{r}, \time)$ is only to regularize and remove density floaters that sit along camera rays that \textit{do not intersect} with any dynamic objects.
% Although it would only be effective in regularizing fuzzy floaters that sit along camera rays that do not hit any dynamic objects, with sufficient camera motion and views from different poses, all spatial locations in the space would be properly reguarlized.

% \AT{nit: if $w(t_b)=1$, there is nothing that promotes $w(t)=0$ between $[0,t_b]$? so this loss is a tad broken? This basically \textit{only} penalizes the existence of floaters for rays that are lucky enough not to hit any object... I guess it doesn't give you a problem because with multiview you have a lot such configurations, in other words the background is a likely ray termination... Perhaps you can defend it with this argument?}
% \WW{Yeah thar's true, this loss does not really help to learn a better dynamic density distribution, but rather just cleans the alpha mask a bit and prevents dynamic component from learning the background. A naive L1 loss on all samples (including those sit along a ray terminated by dynamic object) is likely to lead to a broken dynamic object learned as a thin layer. A better loss for learning good dynamic object would be a density distribution loss like the one below.}

% In theory, the above skewed entropy loss is capable of enforcing a decoupled scene on its own. However, since the skewness in the entropy loss results in a very small gradient as $w$ approaches $0$ (Fig \ref{fig:entropy}), the network has difficulties in converging to a fully decoupled dynamic component, which often includes undesired low-density particles on the background. To increase the robustness and encourage the method to learn the dynamic component with less fuzziness, we apply an L1 loss on the maximum $w$ along each camera ray:  
% 
% \begin{equation}
% L_r(\mathbf{r}) = max_{i=1}^N(w_i)
% \end{equation}
% where $\{w_i\}_{i=1}^N$ is the set of compositing weights of all samples along a ray.
% Intuitively, it encourages dynamic component to occupy as few pixels as possible, while not directly causing a thing-layer-like dynamic object and therefore minimizing the impact on the quality of object learned.
% 

\input{fig/staticentropy}
\paragraph{Static Regularization} 
We empirically found that static component may abuse the camera pose as the hint for the current time frame and learn dynamic effects as sparse clouds that lead to high-frequency appearance changes; see \Figure{static_entropy}.
The ambiguity comes from the fact that we are using monocular casual videos where the camera almost never visits the exact same position twice during the capture.
That is, there exists a one-to-one mapping between camera pose and time variable; see \Figure{shadow_ambiguity}.
We solve this issue by imposing a prior on the distribution of density along a ray, penalizing density distributions that would cause cloud-like artifacts~\cite{infonerf,lolnerf}:
% adapting a density distribution entropy loss on static component~\cite{infonerf}:
% \AT{this is identical to the argument of LoLNeRF? it is a prior on hard (non-fuzzy) surfaces, no?}\WW{Yeah it's a loss with exactly the same effect, just that I knew infoNeRF earlier :)}
% \AT{why not motivate it in the same form then? much easier to explain, no?}
% \WW{I guess the context is slightly different, we probably would want to emphasize why it helps with learning static component in our case? Since we are not exactly doing few-shot/single view training.}
% 
\begin{align}
\mathcal{L}_{\sigma^S}(\mathbf{r}) = - \int_{t_n}^{t_f} p(t) \cdot log \: p(t) \: dt
\quad
\text{where}
\quad
p(t) = \frac{\sigma^S(\mathbf{r}(t))}{ \int_{t_n}^{t_f} \sigma^S(\mathbf{r}(s)) \: ds}
\label{eq:staticentropyloss}
\end{align}
% 
% \begin{equation}
% \begin{split}
% H_{\sigma^S}(\mathbf{r}) &= -\sum_{i=1}^N p_i log \: p_i
% \\
% \text{where } p_i &= \frac{\alpha_i^S}{\sum_{j=1}^N \alpha_j^S}
% \end{split}
% \end{equation}
% \WW{Double check if above sum to integral conversion is correct}
% 
% Intuitively, this can be seen as treating the $\alpha$ values of static component along each ray as a distribution of density, and the entropy loss penalizes the sparse density distribution which leads to cloud-like artifacts, hence improving the quality of scene decoupling and static background reconstruction.
% The above entropy loss regularizes the density distribution along each ray, penalizing uniform distributions that cause cloud-like artifacts and poor background reconstruction.


\subsection{Shadow Fields}
\label{sec:shadows}

While the above formulation can already decouple arbitrary complex dynamic objects involving non-rigid and topological changes, it occasionally fails to correctly explain the shadows of the dynamic objects, especially when the shadows occupy a large area of the scene. Shadow appears to be very challenging to be correctly identified and decoupled due to two reasons: (i) shadow is textureless and is thus naturally ambiguous. Any motion-based decomposition methods can incorrectly identify the bright surface around the shadow as the dynamic effect, accompanied with a darkened static surface (i.e., the bright surface is moving rather then dark shadow is moving); see \Figure{shadow_ambiguity}.
% \FZ{Good place to refer to a figure}
% (ii) Because our method is based on NeRF, a representation that cannot model any radiance effect without occupancy in the space, it is therefore physically incorrect to categorize standalone shadow effects to the dynamic component, which does not have any density and is simply a reduction in the radiance.
(ii) Our method attempts to learn a separation of moving/static scenes by binarily assigning density values to either the dynamic or static NeRF. However, moving shadows are an effect of radiance changes in static scenes which cannot be explained by assigning density values to the dynamic component. 
% Although shadows can be alternatively modeled as a thin, semi-transparent layer of certain physical matter that deforms in every frame, we aim for a physically correct explanation for such effects.
% \WW{I'd avoid such argument (commented out), as in the end we still used shadow decay to model shadow as an "incorrect" representation}


To overcome these issues, we exploit a heuristic that a shadow should always be a reduction in the radiance instead of an increase. We additionally train a shadow field model $\mathcal{F}^\rho$ that maps 3D spatial coordinate and 1D time variable into a shadow ratio $\rho \in \mathbb{R}$, which represents a scale down on the radiance of static component at the same spatial location:
% 
\begin{equation}
\begin{split}
\rho(\mathbf{x}, \time) \in [0,1] = \mathcal{F}^\rho (\mathbf{x}, \time) 
\end{split}
\end{equation}

The composite rendering equation therefore becomes:

\begin{equation}
\begin{split}
% \hat{C}(\mathbf{r}) &= \sum_{i=1}^N T_i(\alpha^S_i\mathbf{c}^S_i (1-\rho_i) + \alpha^D_i\mathbf{c}^D_i)
\hat{C}(\mathbf{r}, \time) = \int_{t_n}^{t_f} T(t)&\left( (1-\rho(\mathbf{r}(t), \tau)) \cdot \sigma^S(t) \cdot \mathbf{c}^S(t)  + \sigma^D(t) \cdot \mathbf{c}^D(t) \right) \, dt
\end{split}
\end{equation}


Note that the emphasis of our method is not on the decoupling of objects and their shadows, but on the disentanglement of dynamic objects and effects from the static background. This formulation of shadow field accounts for shadow cast on static components only. As for shadow on dynamic objects, the dynamic component NeRF would learn it as the time-varying radiance. 

To prevent the shadow field from unnecessarily accounting for static part where a shadow from dynamic component is not cast, we regularize it with an combined loss of L1 and L2:
% as L1 loss ensures sparsity while L2 discourages extremely strong shadow effect, which is usually not realistic.

\begin{equation}
L_\rho (\mathbf{r}) = \frac{1}{N}\sum_{i=1}^N (\rho_i + \rho_i^2)
\end{equation}


\begin{equation}
L_\rho (\mathbf{r}, \time) =  \frac{1}{t_f-t_n} \int_{t_n}^{t_f} \rho(\mathbf{r}(t), \time) + \rho(\mathbf{r}(t), \time)^2 \: dt
\end{equation}

% This loss makes no sense and is removed 
% Additionally, we make a simple assumption that the darkening effects caused by shadow should be similar at the same time stamp. Therefore, we encourage $\rho$ values that are above certain threshold $\gamma$ to be consistent at same frame by penalizing their variance: \TODO{CO: We drop time and space dependency in general, but here we need it to explain.}  

% \begin{equation}
% \begin{aligned}
% L_{\bar{\rho}} &= Var(P) %\frac{1}{\#P}\sum_{\rho \in P} (\rho - \bar{P})
% ,
% \text{where } P = \{\rho | \rho > \gamma\}
% \end{aligned}
% \end{equation}

% We start with low weight for $L_{\bar{\rho}}$ and gradually increase it in the end of training iterations, so that the consistency loss is only effective when the shadow field has introduce enough sparsity.

% \FZ{$\gamma$ is not explained in the text}

\paragraph{Shadow Decay} Because the main objective of our method is to achieve non-rigid dynamic object decoupling, we do not over-extend the method to consider lighting and reflectance decomposition. Without additional knowledge about light source position and accurate static background geometry, there exists uncertainty between the dynamic objects and their shadows. Especially when a dynamic object has similar or darker color to the background, it can be incorrectly explained as a moving shadow cast on the background, leading to significant drop on the quality of novel view synthesis of dynamic object. Therefore, for scenes without significant moving shadows, we gradually increase the weights of $L_\rho$ or directly assign it with a large value to distill the knowledge into the static and dynamic components. At inference time, shadow field is no longer needed and the dynamic component would learn the moving shadows as thin layers with low densities on top of the static surface.




%% version with shadow consistency loss
% The overall loss of our method is:

% \begin{equation}
% \mathcal{L} = \sum_{\mathbf{r} \in \mathcal{R}} \left( (\hat{C}(\mathbf{r}) - C(\mathbf{r}))^2 + \lambda_s H_{s}(\mathbf{r}) + \lambda_r L_r(\mathbf{r}) + \lambda_{\sigma^S} H_{\sigma^S}(\mathbf{r}) + \lambda_\rho L_\rho (\mathbf{r}) \right) + \lambda_{\bar{\rho}} L_{\bar{\rho}}
% \end{equation}

% where $\lambda_s$, $\lambda_r$, $\lambda_{\sigma^S} $, $\lambda_\rho$, $\lambda_{\bar{\rho}}$ are the weights of the regularisation terms respectively.



==> archive.tex <==
\section{Submission of papers to NeurIPS 2021}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2021 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.

The margins in 2021 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2021.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2021 is \verb+neurips_2021.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2021.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2021+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2021}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2021/PaperInformation/FundingDisclosure}.

Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip

{
\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> fig/_abla_shadow.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.75\textwidth]{Figures/abla_shadow.png}
  \caption{Ablation on shadow field component. When the scene presents large area shadows or shadows that move within a small range, the shadow field helps to disentangle them from camera motion and prevents physically unrealistic solution. \WW{merging this to the figure of shadows}}
\end{figure}

==> fig/abla_skew.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{Figures/abla_skew.png}
  \caption{}
  \label{fig:abla_skew}
\end{figure}

==> fig/ablations_shadow.tex <==
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{Figures/ablations_shadow.png}
\captionof{figure}{\textbf{Ablations (shadow) -- }
Our method is able to remove large area of shadows, even if they are strongly correlated with the view direction (e.g., shadow cast by camera or the photographer).
Note that the appearance embedding from NeRF-W \cite{nerfw} is not sufficient to remove shadow that is present throughout the capture.
\AT{remove one row, too many, refer to additional materials for more images}
\AT{reduce font size in column labels (and make single row now)}
}
\label{fig:ablations_shadow}
\end{figure}

==> fig/masks.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\textwidth]{Figures/masks.png}
  \caption{ \textbf{Video segmentation (qualitative) -- }
  MG fails to identify the moving pillow and segments everything out except for the table due to its Hungarian setting. NeRF-W learns the transient component with severe cloud-like effects. While our method achieves best segmentation in all the scenes. }
  \label{fig:masks}
\end{figure}

==> fig/shadow_OLD.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\textwidth]{Figures/shadow.png}
  \caption{With the shadow field, our method is able to remove large area of shadows, even if they are strongly correlated with the view direction (e.g., shadow cast by camera or the photographer).}
\end{figure}

==> fig/static.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\textwidth]{Figures/static.png}
  \caption{ \textbf{Background recovery on synthetic scenes (training views).}
  }
  \label{fig:static}
\end{figure}

==> table/ablations.tex <==
% \begin{table}[h]
% \end{table}

==> table/background_OLD.tex <==
% background recovery novel view =

% no mean version
% \begin{table}[h]
%   \caption{\textbf{Quantitative evaluation on background recovery -- }
% %   Quantitative evaluation on static background recovery task. 
% %   We compared with the baselines and ablations of our method. 
%   We train on each scene with 200 frames, decouple the dynamic objects and shadows, and render the static component from 100 novel views to compare with ground truth. }
%   \centering
%   \setlength\tabcolsep{1.5pt}
%   \tiny
  
%   \begin{tabu}{lccc|ccc|ccc|ccc|ccc}
%     \toprule
%     \multicolumn{1}{c}{}  & \multicolumn{3}{c|}{Car}  & \multicolumn{3}{c|}{Cars} & \multicolumn{3}{c|}{Bag} & \multicolumn{3}{c|}{Chairs} & \multicolumn{3}{c}{Pillow} \\
%     % \cmidrule(r){2-16} 
%     \rowfont{\fontsize{5}{5}\selectfont}
%      & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$\\
%     % \midrule
%     % NeRF-W \cite{nerfw} &  .2176 &  .8144 & 24.2330 &  .2427 &  .8733 & 24.5134 &  .1391 &  .7914 & 20.6475 &  .1500 &  .6809 & 23.7746 &  .0877 &  .9353 & 28.2394    \\
%     % NeuralDiff \cite{neuraldiff}  &  .0646 &  .9518 & 31.8906 &  .0981 &  .9208 & 25.9344 &  .1173 &  .9102 & 29.0247 &  .1118 & \textbf{ .7225} & 24.4249 &  .5646 &  .6517 & 20.0934    \\
%     % \hline
%     % % Ours (template)    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &   \\
%     % Ours (w/o skew)    &  .0615 &  .9745 & 34.3962 &  .1035 &  .9484 & 26.1885 &  .0912 &  .9547 & 31.5461 &  .1506 &  .6528 & 22.9183 &  .1184 &  .9400 & 28.1711  \\
%     % Ours (w/o $L_r$)    &  .2544 &  .8312 & 23.5474 &  .2601 &  .8027 & 22.4660 &  .1888 &  .8930 & 28.3756 &  .1069 &  .6928 & 24.4415 &  .3111 &  .7696 & 15.2721   \\
%     % Ours (w/o skew, $L_r$ )   &  .3146 &  .7917 & 23.0113 &  .1188 &  .9433 & 26.1012 &  .2539 &  .6664 & 19.9591 &  .1042 &  .6978 & 24.4176 &  .3854 &  .6706 & 14.2352   \\
%     % Ours     & \textbf{ .0605} & \textbf{ .9752} & \textbf{34.4962} & \textbf{ .0904} & \textbf{ .9534} & \textbf{26.2675} & \textbf{ .0764} & \textbf{ .9788} & \textbf{34.1404} & \textbf{ .0949} &  .7069 & \textbf{24.6340} & \textbf{ .0762} & \textbf{ .9789} & \textbf{36.5835}     \\
%     % \bottomrule
%     \midrule
%     NeRF-W \cite{nerfw} &  .218 &  .814 & 24.23 &  .243 &  .873 & 24.51 &  .139 &  .791 & 20.65 &  .150 &  .681 & 23.77 &  .0877 &  .935 & 28.24    \\
%     NeuralDiff \cite{neuraldiff}  &  .0646 &  .952 & 31.89 &  .0981 &  .921 & 25.93 &  .117 &  .910 & 29.02 &  .112 & \textbf{ .722} & 24.42 &  .565 &  .652 & 20.09    \\
%     \hline
%     % Ours (template)    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &   \\
%     Ours (w/o skew)    &  .0615 &  .974 & 34.40 &  .104 &  .948 & 26.19 &  .0912 &  .955 & 31.55 &  .151 &  .653 & 22.92 &  .118 &  .940 & 28.17  \\
%     Ours (w/o $L_r$)    &  .254 &  .831 & 23.55 &  .260 &  .803 & 22.47 &  .189 &  .893 & 28.38 &  .107 &  .693 & 24.44 &  .311 &  .770 & 15.27   \\
%     Ours (w/o skew, $L_r$ )   &  .315 &  .792 & 23.01 &  .119 &  .943 & 26.10 &  .254 &  .666 & 19.96 &  .104 &  .698 & 24.42 &  .385 &  .671 & 14.24   \\
%     Ours     & \textbf{ .0605} & \textbf{ .975} & \textbf{34.50} & \textbf{ .0904} & \textbf{ .953} & \textbf{26.27} & \textbf{ .0764} & \textbf{ .979} & \textbf{34.14} & \textbf{ .0949} &  .707 & \textbf{24.63} & \textbf{ .0762} & \textbf{ .979} & \textbf{36.58}     \\
%     \bottomrule
%   \end{tabu} \label{table:background}
% \end{table}


% background recovery novel view =

\begin{table}[h]
\caption{\textbf{Scene decoupling -- }
We train on each scene with 200 frames, decouple the dynamic objects and shadows, and render the static component from 100 novel views to compare with ground truth.
}
  \centering
  \setlength\tabcolsep{1.5pt}
  \resizebox{\linewidth}{!}{
  \begin{tabu}{lccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{3}{c|}{Car}  & \multicolumn{3}{c|}{Cars} & \multicolumn{3}{c|}{Bag} & \multicolumn{3}{c|}{Chairs} & \multicolumn{3}{c}{Pillow}& \multicolumn{3}{c}{Mean} \\
    % \cmidrule(r){2-16} 
    \rowfont{\fontsize{4}{5}\selectfont}
     & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$\\
    
    \midrule
    NeRF-W \cite{nerfw} &  .218 &  .814 & 24.23 &  .243 &  .873 & 24.51 &  .139 &  .791 & 20.65 &  .150 &  .681 & 23.77 &  .0877 &  .935 & 28.24 & .167 & .819 & 24.28     \\
    NeuralDiff \cite{neuraldiff}  &  .0646 &  .952 & 31.89 &  .0981 &  .921 & 25.93 &  .117 &  .910 & 29.02 &  .112 & \textbf{ .722} & 24.42 &  .565 &  .652 & 20.09 & .191 & .831 & 26.27     \\
    \hline
    % Ours (template)    &  &  &  &  &  &  &  &  &  &  &  &  &  &  &   \\
    Ours (w/o skew)    &  .0667 &  .973 & 34.06 &  .104 &  .948 & 26.19 &  .0912 &  .955 & 31.55 &  .151 &  .653 & 22.92 &  .118 &  .940 & 28.17 & .106 & .894 & 28.58   \\
    Ours (w/o $L_r$)    &  .182 &  .865 & 25.89 &  .260 &  .803 & 22.47 &  .189 &  .893 & 28.38 &  .107 &  .693 & 24.44 &  .311 &  .770 & 15.27 & .210 & .805 & 23.29    \\
    Ours (w/o skew, $L_r$ )   &  .214 &  .834 & 26.26 &  .119 &  .943 & 26.10 &  .254 &  .666 & 19.96 &  .104 &  .698 & 24.42 &  .385 &  .671 & 14.24 & .215 & .762 & 22.20    \\
    Ours     & \textbf{ .0615} & \textbf{ .975} & \textbf{34.27} & \textbf{ .0904} & \textbf{ .953} & \textbf{26.27} & \textbf{ .0764} & \textbf{ .979} & \textbf{34.14} & \textbf{ .0949} &  .707 & \textbf{24.63} & \textbf{ .0762} & \textbf{ .979} & \textbf{36.58} & \textbf{.0799} & \textbf{.919} & \textbf{31.18}      \\
    \bottomrule
  \end{tabu} \label{table:background}
  } % \resizebox
\end{table}

==> table/background_train.tex <==


\begin{table}[H]
  \caption{Static Background Recovery (training views) \WW{this goes to appendix}}
  \centering
  \setlength\tabcolsep{1.5pt}
  \tiny
  \begin{tabular}{cccc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{3}{c|}{Car}  & \multicolumn{3}{c|}{Cars} & \multicolumn{3}{c|}{Bag} & \multicolumn{3}{c|}{Chairs} & \multicolumn{3}{c}{Pillow} \\
    % \cmidrule(r){2-16} 
     & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$\\
    \midrule
    NeRF-W \cite{nerfw} & 0.1904 & 0.8442 & 24.9042 & 0.2090 & 0.9115 & 31.3062 & 0.1398 & 0.7978 & 20.8200 & 0.0508 & 0.9606 &  33.6986 & 0.0614 & 0.9577 & 29.0613   \\
    NeuralDiff \cite{neuraldiff}  & \textbf{0.0233} & \textbf{0.9896} & \textbf{38.1582} & \textbf{0.0320} & \textbf{0.9875} & \textbf{38.2171} & 0.1104 & 0.9264 & 29.7108 & 0.0495 & 0.9776 & 36.1120 & 0.5330 & 0.7718 & 20.7323      \\
    
    Ours     & 0.0552 & 0.9838 & 35.5181 & 0.0621 & 0.9780 & 35.1081 & \textbf{0.0799} & \textbf{0.9805} & \textbf{34.6348} & \textbf{0.0354} & \textbf{0.9834} & \textbf{36.9118} & \textbf{0.0659} & \textbf{0.9868} & \textbf{38.4760}     \\
    \bottomrule
  \end{tabular}
\end{table}

==> table/background_train_val.tex <==
\begin{table}[H]
  \centering
    \caption{Quantitative evaluation on static background recovery task. Each scene is consisted of 200 frames of static background captured from training views and additional 100 frames of unseen novel views. See the supplement for a breakdown comparison on training and novel views. \WW{this goes to appendix}}
  \setlength\tabcolsep{1.5pt}
  \tiny
  \begin{tabular}{cccc|ccc|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{3}{c|}{Car}  & \multicolumn{3}{c|}{Cars} & \multicolumn{3}{c|}{Bag} & \multicolumn{3}{c|}{Chairs} & \multicolumn{3}{c}{Pillow} \\
    % \cmidrule(r){2-16}
     & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$\\
    \midrule
    NeRF-W \cite{nerfw} & 0.1994 & 0.8343 & 24.6804 & 0.2202 & 0.8988 & 29.0419 & 0.1395 & 0.7957 & 20.7625 & 0.0839 & 0.8674 & 30.3906 & 0.0702 & 0.9502 & 28.7874 \\
    NeuralDiff \cite{neuraldiff}  & \textbf{0.0371} & 0.9770 & \textbf{36.0690} & \textbf{0.0540} & 0.9653 & \textbf{34.1228} & 0.1127 & 0.9210 & 29.4821 & 0.0703 & \textbf{0.8925} & 32.2163 & 0.5435 & 0.7318 & 20.5194      \\
    
    Ours     & 0.0569 & \textbf{0.9809} & 35.1775 & 0.0715 & \textbf{0.9698} & 32.1612 & \textbf{0.0787} & \textbf{0.9799} & \textbf{34.4700} & \textbf{0.0552} & 0.8913 & \textbf{32.8192} & \textbf{0.0693} & \textbf{0.9842} & \textbf{37.8451}     \\
    \bottomrule
  \end{tabular}
 \end{table}

==> table/novel_view_synthetic.tex <==
\begin{table}[H]
  \caption{Novel view synthesis on synthetic dataset (this probably goes to appendix)}
  \centering
  \setlength\tabcolsep{2pt}
  \tiny
  \begin{tabular}{cccccccccccccccc}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{3}{c}{Car}  & \multicolumn{3}{c}{Cars} & \multicolumn{3}{c}{Bag} & \multicolumn{3}{c}{Chairs} & \multicolumn{3}{c}{Pillow}        \\
    \cmidrule(r){2-16} 
     & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$\\
    \midrule
    HN(base) &     \\
    HN(fair) &     \\
    
    Ours     & 0.1439 & 0.8870 & 24.906 & 0.1759 & 0.8649 & 23.980 & 0.0903 & 0.9618 & 31.233 & 0.1094 & 0.9054 & 27.336 & 0.1051 & 0.9506 & 31.156    \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[H]
  \caption{Novel view synthesis on all dataset}
  \centering
  \setlength\tabcolsep{2pt}
  \tiny
  \begin{tabular}{cccccccccccccccccccccccccccc}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{3}{c}{Broom}  & \multicolumn{3}{c}{Printer} & \multicolumn{3}{c}{Chicken} & \multicolumn{3}{c}{Banana} & \multicolumn{3}{c}{Pick}  & \multicolumn{3}{c}{Duck} & \multicolumn{3}{c}{Balloon} & \multicolumn{3}{c}{Water}  & \multicolumn{3}{c}{Cookie}       \\
    \cmidrule(r){2-28} 
     & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$ & LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$& LPIPS$\downarrow$ & MS-SSIM$\uparrow$ & PNSR$\uparrow$\\
    \midrule
    HN(base) & 0.5243 & 0.6355 & 19.653 & 0.2134 & 0.7817 & \textbf{19.889} & 0.2221 & 0.8775 & 23.940 & 0.2227 & 0.8184 & 21.205 & 0.4956 & 0.4132 & 13.064 & 0.2511 & 0.8299 & 20.639 & 0.1954 & 0.8028 & 17.808 & 0.3599 & 0.4829 & 15.065 & 0.1612 & 0.8360 & 19.930 \\
    
    HN(fair) & \textbf{0.5029} & 0.6242 & 19.377 & \textbf{0.1959} & \textbf{0.7819} & 19.797 & \textbf{0.1800} & 0.8809 & 23.680 & \textbf{0.1944} & \textbf{0.8322} & 21.525 & 0.4855 & 0.4093 & 13.143 & 0.2531 & 0.8183 & 20.320 & 0.1868 & 0.8043 & 17.920 & 0.3608 & 0.4648 & 14.802 & 0.1619 & 0.8011 & 19.750\\
    
    Ours     & 0.5647 & \textbf{0.7120} & \textbf{20.656} & 0.2240 & 0.7775 & 19.749 & 0.2036 & \textbf{0.8904} & \textbf{24.274} & 0.2536 & 0.8283 & \textbf{21.593} & \textbf{0.2532} & \textbf{0.8249} & \textbf{20.318} & \textbf{0.2321} & \textbf{0.8391} & \textbf{21.459} & \textbf{0.1528} & \textbf{0.8579} & \textbf{20.925} & \textbf{0.1531} & \textbf{0.8492} & \textbf{21.628} & \textbf{0.1519} & \textbf{0.8805} & \textbf{20.293}  \\
    \bottomrule
  \end{tabular}
\end{table}

==> table/placeholder.tex <==
\centering
\setlength\tabcolsep{1.5pt}
\tiny
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{1}{c}{}  & \multicolumn{1}{c|}{Car}  & \multicolumn{1}{c|}{Cars} & \multicolumn{1}{c|}{Bag} & \multicolumn{1}{c|}{Chairs} & \multicolumn{1}{c|}{Pillow}  & \multicolumn{1}{c}{Mean}        \\
% \cmidrule(r){2-13} 
 & $\mathcal{J}\uparrow$ &   $\mathcal{J}\uparrow$ &   $\mathcal{J}\uparrow$ &   $\mathcal{J}\uparrow$ &   $\mathcal{J}\uparrow$ &   $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$\\


\midrule
MG \cite{motiongroup} &  .603 &   .363 &   .629 &   .484 &   .0436 &   .424  \\
NeRF-W \cite{nerfw} &  .0719 &  .0979 &  .0273 &  .154 &  .194 &  .109 & \\
NeuralDiff \cite{neuraldiff}     &  .806 &  .508 &  .0803 &  .368 &  .0972 &  .372 &  \\
\hline
Ours     &  \textbf{.848} &   .790 &  \textbf{ .703} & \textbf{ .551} & \textbf{ .693 }& \textbf{ .717} &    \\
\bottomrule
\end{tabular}
} % \resizebox

==> table/seg.tex <==
\begin{table}[ht]
% \begin{wraptable}{L}{0.6\textwidth}
\caption{\textbf{Video segmentation --}
% \AT{isn't this video segmentation more than image?}
We report Jaccard index $\mathcal{J}$ and boundary measure $\mathcal{F}$ on training views. Our method performs well on "car" and "cars" dataset without use of skewed entropy because the background is clearly distinguishable from the moving object.}
  \centering
  \setlength\tabcolsep{1.5pt}
  \tiny
%   \resizebox{\linewidth}{!}{ % resizebox causes font to be too big, just stick with /tiny probably
  \begin{tabular}{lcc|cc|cc|cc|cc|cc}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{2}{c|}{Car}  & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Bag} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Pillow}  & \multicolumn{2}{c}{Mean}        \\
    % \cmidrule(r){2-13} 
     & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$  & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$  & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$  & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$  & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$  & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$\\
    % \midrule
    % MG \cite{motiongroup} &  .6031 &  .7432 &  .3629 &  .4738 &  .6293 &  .7378 &  .4839 &  .6126 &  .0436 &  .0798 &  .4245 &  .5294 \\
    % NeRF-W \cite{nerfw} &  .0719 &  .1325 &  .0979 &  .1622 &  .0273 &  .0525 &  .1539 &  .2541 &  .1940 &  .3135 &  .1090 &  .1829 \\
    % NeuralDiff \cite{neuraldiff}     &  .8062 &  .8909 &  .5085 &  .5777 &  .0803 &  .1445 &  .3678 &  .5133 &  .0972 &  .1769 &  .3720 &  .4607  \\
    
    % \hline
    
    % Ours (w/o skew) & \textbf{ .8830} & \textbf{ .9377} & \textbf{ .8072} & \textbf{ .8830} &  .3418 &  .4831 &  .1140 &  .1977 &  .3472 &  .5112 &  .4986 &  .6025\\
    % Ours (w/o $L_r$) &  .0544 &  .1023 &  .1742 &  .2614 &  .0475 &  .0886 &  .2370 &  .3670 &  .0405 &  .0779 &  .1107 &  .1794\\
    % Ours (w/o skew, $L_r$) &  .0562 &  .1056 &  .3765 &  .4640 &  .0433 &  .0812 &  .3148 &  .4527 &  .0272 &  .0529 &  .1636 &  .2313\\
    
    % Ours     &  .8630 &  .9262 &  .7902 &  .8735 & \textbf{ .7031} & \textbf{ .8177} & \textbf{ .5511} & \textbf{ .6867} & \textbf{ .6931 }& \textbf{ .8182} & \textbf{ .7201} & \textbf{ .8244}    \\
    % \bottomrule
    
    \midrule
    MG \cite{motiongroup} &  .603 &  .743 &  .363 &  .474 &  .629 &  .738 &  .484 &  .613 &  .044 &  .080 &  .424 &  .529 \\
    NeRF-W \cite{nerfw} &  .072 &  .132 &  .098 &  .162 &  .027 &  .052 &  .154 &  .254 &  .194 &  .314 &  .109 &  .183 \\
    NeuralDiff \cite{neuraldiff}     &  .806 &  .891 &  .508 &  .578 &  .080 &  .144 &  .368 &  .513 &  .097 &  .177 &  .372 &  .461  \\
    \hline
    Ours (w/o skew) & .814 & .896 & \textbf{ .807} & \textbf{ .883} &  .342 &  .483 &  .114 &  .198 &  .347 &  .511 &  .485 &  .594\\
    Ours (w/o $L_r$) &  .076 &  .139 &  .174 &  .261 &  .048 &  .089 &  .237 &  .367 &  .040 &  .078 &  .115 &  .187\\
    Ours (w/o skew, $L_r$) &  .077 &  .142 &  .376 &  .464 &  .043 &  .081 &  .315 &  .453 &  .027 &  .053 &  .168 &  .238\\
    Ours     &  \textbf{.848} &  \textbf{.917} &  .790 &  .874 & \textbf{ .703} & \textbf{ .818} & \textbf{ .551} & \textbf{ .687} & \textbf{ .693 }& \textbf{ .818} & \textbf{ .717} & \textbf{ .822}    \\
    \bottomrule
  \end{tabular}\label{table:seg}
%   }
% \end{wraptable}
\end{table}

